Prioritize Alignment in Dataset Distillation

Dataset Distillation aims to compress a large dataset into a significantly more compact, synthetic one without compromising the performance of the trained models. To achieve this, existing methods use the agent model to extract information from the target dataset and embed it into the distilled dataset. Consequently, the quality of extracted and embedded information determines the quality of the distilled dataset. In this work, we find that existing methods introduce misaligned information in both information extraction and embedding stages. To alleviate this, we propose Prioritize Alignment in Dataset Distillation (PAD), which aligns information from the following two perspectives. 1) We prune the target dataset according to the compressing ratio to filter the information that can be extracted by the agent model. 2) We use only deep layers of the agent model to perform the distillation to avoid excessively introducing low-level information. This simple strategy effectively filters out misaligned information and brings non-trivial improvement for mainstream matching-based distillation algorithms. Furthermore, built on trajectory matching, \textbf{PAD} achieves remarkable improvements on various benchmarks, achieving state-of-the-art performance.

==> sec/1_introduction_v2.tex <==
\section{Introduction}

Dataset Distillation (DD)~\cite{wang2020dataset} aims to compress a large dataset into a small synthetic dataset that preserves important features for models to achieve comparable performances. Recently, matching-based methods have shown prominent capabilities for distilling high-quality synthetic datasets. These methods minimize a specific metric learned from the synthetic data and target data, including gradients~\cite{Zhao2020DatasetCW, Zhang2023DatasetCV}, distributions~\cite{Zhao2023ImprovedDM}, and training trajectories~\cite{Cazenavette2022DatasetDB, Guo2023TowardsLD}.


The core idea of matching-based methods can be summarized as follows: Firstly, a surrogate model is trained on the real data to learn the information of the target dataset. Secondly, learned information is embedded into the synthetic dataset through metric matching. However, we find that both steps introduce noisy information to the synthetic dataset. In this work, we use trajectory matching (TM) methods to demonstrate why noisy information exists and propose our method to purify the dataset distillation process.


Introduced by~\cite{Arpit2017ACL}, deep neural networks (DNNs) typically learn to recognize easy patterns early in training and hard patterns later on. Therefore, DATM~\cite{Guo2023TowardsLD} proposes to tune the matching range in accordance with the changes in IPC. 
Specifically, small IPCs should match early trajectories to distill easy patterns, while larger IPCs match late trajectories to distill harder ones.
However, we argue that the difficulty alignment is not conducted from the source. 
As illustrated in Figure~\ref{fig: method}, when training expert trajectories, existing methods allow the surrogate model to see all samples in the target dataset~\cite{Cazenavette2022DatasetDB, Du2022MinimizingTA} at every single epoch, which enables the model to learn hard(easy) information at early(late) trajectories.
This difficulty misaligned information manifests as noise in the later trajectory matching phase.


Currently, TM methods use all parameters of the surrogate model to compute the distance between expert and student trajectories. 
However, different layers of a DNN learn different representations of the input data.
Previous studies on the interpretability of convolutional neural networks~\cite{Mahendran2016VisualizingDC, Selvaraju2016GradCAMVE} demonstrate a key finding that as layers progress deeper into the network, they encode higher-level content of the image, moving from general information such as color in the shallow layers to more detailed and semantic information in deeper layers. 
As IPC increases, it is trivial for the distilled dataset to contain sufficient simple patterns and more hard patterns are needed to achieve better performance. 
Therefore, ignorance of representation differences between different layers results in excessively matching the trajectory of shallow layers, which only injects low-level noisy information.


Motivated by the above analysis, we propose XXX to filter out noisy information from the two sources. 
To filter learned information by surrogate models, we employ data selection methods to measure the difficulty of each sample in the original dataset. Then, by meticulously designing a training data scheduler, we are able to flexibly control the difficulty of data the model is trained on at different training phases. 
To filter distilled information during trajectory matching, we propose parameter selection, given that matching shallow-layer parameters doesn't contribute to distilling representative features. 
Specifically, we discard a pre-defined ratio of shallow-layer parameters and only use the rest of deep-layer parameters to calculate the trajectory distance. This is especially effective on larger IPCs as they require more high-level information.


Our proposed method brings non-trivial improvements to existing TM methods~\cite{Cazenavette2022DatasetDB, Du2022MinimizingTA, Guo2023TowardsLD} across several well-known benchmarks. We achieve new state-of-the-art results on both small and large IPCs. Our distilled dataset also possesses good generalizability on unseen neural network architectures. Notably, although XXX is built upon TM-based methods, it can generalize well to other matching-based methods, such as matching gradients and matching distributions. Two filtering modules can both bring improvements on other matching-based algorithms (see results in ...). 





















\iffalse

%第一段：简单介绍背景，定义我们要解决的问题
%zhiqi：先介绍DD的核心思想，再列举其应用效果和重要性。
Dataset Distillation (DD)~\cite{wang2020dataset} aims to compress a large dataset into a small synthetic dataset, such that models trained on this condensed dataset can achieve performance comparable to those trained on the original dataset. 
So far, dataset distillation not only achieved great success when the compression ratio is extremely high \cite{Cazenavette2022DatasetDB, Zhao2020DatasetCW}, but also can achieve lossless performance for model training \cite{Guo2023TowardsLD}.
Due to its effectiveness, dataset distillation has been widely applied in practical fields such as privacy preservation~\cite{Dong2022PrivacyFF, Yu2023MultimodalFL}, continual learning \cite{masarczyk2020reducing, rosasco2021distilled}, and neural architecture search~\cite{Jin2018AutoKerasAE, Pasunuru2019ContinualAM}.

Generally, the process of most dataset distillation algorithms can be divided into two steps: (1) use a surrogate model to learn the information of the target dataset,
(2) embed the learned information into the synthetic dataset.
In practice, step (1) is realized by recording several metrics calculated by a surrogate model on the target dataset, such as gradients \cite{Zhao2020DatasetCW, Zhang2023DatasetCV}, distributions \cite{Zhao2021DatasetCW1}, and training trajectories \cite{Cazenavette2022DatasetDB, Guo2023TowardsLD}.
Then, in step (2), the synthetic data is optimized such that the same metrics calculated on the distilled dataset become similar to the ones recorded in step (1).

Through the above two steps, information important for the model training will be extracted and embedded into the synthetic data.
However, in this work, we show these two steps both will introduce unnecessary noisy information to the synthetic data, harming the performance of distilled datasets.

In the first step, to extract information, the distillation algorithms use the surrogate model to calculate several metrics based on data points randomly sampled from the target dataset \cite{Zhao2020DatasetCW, Zhao2021DatasetCW1, Cazenavette2022DatasetDB}.
In other words, here the surrogate model gets the chance to see all data samples of the target dataset. 
However, not all samples can provide useful information, since information that helps to learn basic distribution is only needed when the compression ratio is extremely high \cite{ Guo2023TowardsLD}.
Through experiments, we find selecting data points based on their difficulties for models to learn can prevent the surrogate model from learning harmful information in the first step, purring the information embedded into the synthetic dataset.

In the second step, distillation algorithms always use \textbf{all} parameters of the surrogate model to calculate the pre-defined metrics on the synthetic dataset \cite{Zhao2020DatasetCW, Cazenavette2022DatasetDB, Guo2023TowardsLD, Wang2022CAFELT}, which are then used to match the one obtained in step (1) to embed the extracted information into the synthetic data.
However, we show that matching metrics calculated by parameters from shallow layers of the surrogate model provide low-quality noisy information, while parameters from deep layers provide high-level semantical information.
These results are consistent with previous findings that show deeper layers in DNNs focus on higher-level and more general features of input \cite{Mahendran2016VisualizingDC, Selvaraju2016GradCAMVE}.
To avoid introducing noisy information to the distilled datasets, we propose to use only deeper layer of surrogate models to perform the distillation.

% However, one significant limitation of these algorithms is that not all information is useful for achieving good performance, and useless information is also distilled into synthetic images.
% In this work, we empirically find useless information comes from two sources: information learned by surrogate models from the target dataset and information distilled by matching parameters of surroagte models. Thus, we propose two filter modules to refine these two sources separately.
%zhiqic:提升下和上段之前的过度。
% An insightful observation introduced by DATM~\citep{Guo2023TowardsLD} is that the student model shows a tendency to learn easy patterns at the early stage of the trajectory and harder ones later. However, current expert trajectory training simply uses the full dataset and doesn't control the difficulty of information that the expert model sees at different stages of the training trajectory. This results in expert models extracting hard patterns at the early trajectory and easy patterns at the late trajectory. Consequently, this inconsistent information appears as noises that affect difficulty-aligned trajectory matching.

%zhiqi:这里应该大量的引用之前的工作来支持自己的结论
% Based on discoveries of previous works~\cite{Arpit2017ACL, Liu2023DREAMED, Guo2023TowardsLD}, distilling different IPCs requires information of various difficulty levels. This also implies that the surrogate model is expected to learn different information at different training phases. However, current methodologies in surrogate model training on the original dataset indiscriminately utilize the full dataset without modulating the difficulty of information presented to the model at various training stages. Take trajectory matching as an example. The current training strategy leads to the extraction of hard information at the early stages and the preservation of easy information at the late trajectory. Such inconsistencies manifest as useless information that adversely impacts the distilled data. (see section ~\ref{method:fli})


%zhiqic: 1.这里要对应到实验部分的结果。2. 最好要有具体的数值。
% Existing matching-based DD methods follow a similar workflow that matches some specific parameters of surrogate models trained on the original and synthetic datasets~\cite{Zhao2020DatasetCW, Zhao2023ImprovedDM, Cazenavette2022DatasetDB}. However, the ignorance of differences between information distilled by matching parameters from different layers causes the injection of useless information into the distilled data. Previous studies on the interpretability of convolutional neural networks~\cite{Mahendran2016VisualizingDC, Selvaraju2016GradCAMVE} demonstrate a key finding that as layers progress deeper into the network, they encode higher-level content of the image, moving from general content and color in the shallow layers to more detailed and specific content in deeper layers. Our empirical findings (see section~\ref{method:fdi}) show that matching parameters from different layers of the student model inject different features into the synthetic images. Specifically, matching shallow-layer parameters only distills low-level basic image features into the synthetic data. Basic information, however, is likely to be class-irrelevant. By contrast, more useful information that contributes to classification is obtained by matching deep-layer parameters.

% 第四段：提出我们的方法，是分别从这两部分入手，对于教师路径训练，我们提出课程学习，用滑动窗口的方式控制训练数据的难度；对于student模型，我们提出冻住低层参数，只匹配高层参数。（这里要画个图）

Our filtering information in two steps strategy is useful for almost all dataset distillation algorithms including methods based on matching distribution \cite{Zhao2021DatasetCW1, Wang2022CAFELT, Zhao2023ImprovedDM}, gradients \cite{Zhao2020DatasetCW}, and training trajectories \cite{Cazenavette2022DatasetDB, Guo2023TowardsLD}, bringing non-trivial performance improvement.
Moreover, by applying our strategy on trajectory matching \cite{Cazenavette2022DatasetDB, Guo2023TowardsLD}, our novel method called XXXXX achieves state-of-the-art performance on various benchmarks.

% The above analysis motivates us to filter useless information distilled into synthetic data from the two sources.
% To filter learned information by surrogate models, we employ data selection methods to measure the difficulty of each sample in the original dataset. Then, by meticulously designing a training data scheduler, we are able to flexibly control the distribution of data difficulty at different training phases. Given that matching shallow-layer parameters doesn't contribute to distilling useful information, we only use parameters of deeper layers to do the matching. This is especially effective on larger IPCs as they require more high-level information.  

% Our proposed method is effective on all existing matching-based DD algorithms, including matching gradients, distributions, and trajectories. Compared with state-of-the-art (SOTA) results achieved by trajectory matching, XXX brings remarkable improvements on well-known benchmarks and achieves new SOTA on large IPCs.

\fi

==> sec/8_limitation.tex <==
\section{Limitations}
Our data and parameter alignment strategy could be applied to methods based on matching distributions \ref{appendix dm}, gradients \ref{appendix dc}, and training trajectories \ref{appendix mtt}.
However, due to the limitation of computing resources, for methods based on matching distributions and gradients, we only evaluate our method's performance on a few benchmarks.
